Privacy and Accuracy-Aware AI/ML Model Deduplication

With the growing adoption of privacy-preserving machine learning algorithms, such as Differentially Private Stochastic Gradient Descent (DP-SGD), training or fine-tuning models on private datasets has become increasingly prevalent. This shift has led to the need for models offering varying privacy guarantees and utility levels to satisfy diverse user requirements. However, managing numerous versions of large models introduces significant operational challenges, including increased inference latency, higher resource consumption, and elevated costs. Model deduplication is a technique widely used by many model serving and database systems to support high-performance and low-cost inference queries and model diagnosis queries. However, none of the existing model deduplication works has considered privacy, leading to unbounded aggregation of privacy costs for certain deduplicated models and inefficiencies when applied to deduplicate DP-trained models. We formalize the problems of deduplicating DP-trained models for the first time and propose a novel privacy- and accuracy-aware deduplication mechanism to address the problems. We developed a greedy strategy to select and assign base models to target models to minimize storage and privacy costs. When deduplicating a target model, we dynamically schedule accuracy validations and apply the Sparse Vector Technique to reduce the privacy costs associated with private validation data. Compared to baselines that do not provide privacy guarantees, our approach improved the compression ratio by up to $35\times$ for individual models (including large language models and vision transformers). We also observed up to $43\times$ inference speedup due to the reduction of I/O operations.

==> basemodel1.tex <==
{\color{black}
\vspace{-5pt}
\subsection{Base Model Selection}
\label{sec:base-model}
\subsubsection{Problem Analysis and Formalization}
% \textcolor{blue}{Hong: consider introduce a dummy model as the base model, to answer the question of how to choose a base model. The general idea is that we first group the models by their training dataset and model architecture, then come to the point of our current model deduplication algorithm. We can add an experiment to show how to choose the privacy budget to train a dummy base model. In other parts of the paper, we just assume that a dummy model is already selected.}
%The nature of the optimization problem formalized in Sec.~\ref{sec:formulation} is to balance the compression ratio (i.e., the optimization goal) and the constraints on privacy budget increases and utility drops. 
As mentioned, the base models represent the source models that provide blocks for deduplicating a target model, and these models are selected from the models managed by the underlying infrastructure. According to the privacy analysis, the more base models, the higher the privacy budget increase will result for the target model, which is the \textbf{key factor} to meet the privacy budget requirements.  %\textcolor{blue}{We first present some properties of base model selection and their implications in the form of QA, then describe a local strategy based on the properties. Lastly, we propose a global strategy as an improvement over the local strategy to address the fairness constraint.} 
%\epsilon'_t = \max(\epsilon_t, \hat{\epsilon})$, if $R(M_t)\neq R(\hat{M})
Using a base model $\hat{M}$ to deduplicate a target model $M_t$ by transforming it to $M'_t$. With $R(\cdot)$ to denote the training dataset identifier of the input model, $M'_t$'s privacy budget change is 
\begin{equation}
\label{eq-1}
\begin{cases}
\epsilon'_t = \epsilon_t+\hat{\epsilon}, \quad \text{if}\quad R(M_t)=R(\hat{M})\\
\epsilon'_t = \max(\epsilon_t, \hat{\epsilon}), \quad\text{if}\quad R(M_t)\neq R(\hat{M})
\end{cases}
\end{equation}
Target model $M_t$'s privacy budget increase $\Delta\epsilon_t \triangleq \epsilon'_t -\epsilon_t$ must be less than its threshold $\epsilon^*_t$, denoted as follows: %so that the maximum privacy budget increase across datasets meets the constraint.
% \textbf{Q2. How do base models control the privacy budget?} Constraining the increase in the privacy budget in the target model requires constraining the sum of the privacy budget of base models trained on the same dataset according to Theorem~\ref{privacy-with-deduplication}. 

\begin{equation}
\begin{cases}
\label{eq:eq1}
\hat{\epsilon} < \epsilon^* &\qquad\text{if}\quad R(M)=R(\hat{M_t})\\
\hat{\epsilon} < \epsilon_t + \epsilon^* &\qquad\text{if}\quad R(M_t)\neq R(\hat{M})
\end{cases}
\end{equation}

%Given a target model and a privacy budget increase threshold, more than one combination of models may qualify as base models. 


A key question is how to assign the base models for each target model to maximize the compression ratio while meeting the privacy budget increase threshold.  We start from the assumption that we do not allow any model to be used as base model and target model at the same time since deduplicating a model $M_i$ as a target model will lead to parameter and accuracy changes in the models that were deduplicated using $M_i$ as a base model. We define the problem as follows and then we will show that the problem is a \textit{black-box weighted max-cut problem}. 

\noindent
\textbf{Problem Definition.} Given a set of models, $\mathcal{M}=\{M_1, ..., M_n\}$, and the utility drop threshold $t_i^*$ for $M_i$, we suppose $n_{ij}$ represents the number of blocks from $M_j$ that can be replaced by blocks from $M_i$ with $M_j$'s utility drop bounded by $t_j^*$. Here, $M_i$ is the base model and $M_j$ is the target model. The goal is to assign the set of models $\mathcal{M}$ to $n$ deduplication groups, with the $i$-th deduplication group specifying the target models using $M_i$ as the base model, so that $x_{ij} = 1$ means $M_j$ is assigned to the $i$-th group, or in other words, $M_j$ is assigned as a target model of the base model $M_i$. %Furthermore, $a_{ij} =\frac{|\mathcal{G}_i \cap \mathcal{G}_j|}{|\mathcal{G}_i \cup \mathcal{G}_j|}$ represents the Jaccard Similarity between the sets of base models in the $i$-th group (i.e., $\mathcal{G}_i$) and the $j$-th group (i.e., $\mathcal{G}_j$). 
In summary, $\mathcal{X}=\{x_{ij}\}$ is the assignment matrix that assigns target models to each base model's deduplication groups, $\mathcal{N}=\{n_{ij}\}$ is to measure the potential benefit of deduplicating two models. 

In addition, the assignment must meet the privacy budget increase constraint specified in Eq.~\ref{eq:eq1}. Furthermore, models trained on the same dataset for the same task are subject to the fairness constraint specified in Eq.~\ref{eq:fairness}. We meet this constraint by ensuring that the ordering of utilities and privacy budgets for these models do not change after deduplicating all models subject to the fairness constraint. If the utility of $M_i$ is smaller than $M_{i+1}$ ($u_i > u_{i+1}$), and if the user-specified acceptable utility ranges of $M_{i}$ and $M_{i+1}$ after deduplication overlap with each other, i.e., $u_i - t_i^* < u_{i+1} - t_{i+1}^*$, it is possible that the utility of $M_i$ after deduplication is less than the utility of $M_{i+1}$ after deduplication ($u'_i < u'_{i+1}$), which violates the ordering. To ensure the ordering, we reduce the user-specified utility drop threshold $t_i^*$ to be $t_i^{adjusted}=min(t_i^*, u_{i+1}-u_{i})$ so that $M_i$'s new utility is always greater than the next model $M_{i+1}$'s original utility. Similarly, we adjust (i.e. reduce) the user-specified privacy budget increase threshold so that $\epsilon_i^{adjusted}=min(\epsilon_i^*, \epsilon_{i}-\epsilon_{i+1})$. 
%(In Sec.~\ref{sec:greedy}, we will discuss whether it is possible to relax these constraints using a dynamic base model selection algorithm with total ordering.) 
With these constraints, the problem can be formalized as follows:

\begin{equation}
\label{eq:basemodel-selection}
\underset{x_{ij}(1 \leq i,j \leq n)}{\max}\sum\limits_{i=1}^{n}\sum\limits_{j=1}^{n}{n_{ij}\times{x_{ij}}}, \quad s.t.
\end{equation}
\begin{equation}
\label{eq:problem_constraint}
\begin{cases}
{\epsilon}_i < \epsilon^{adjusted}_j &\qquad\text{if}\quad R(M)=R(\hat{M_t}) \wedge x_{ij}=1\\
{\epsilon}_i < \epsilon_j + \epsilon^{adjusted}_j &\qquad\text{if}\quad R(M_t)\neq R(\hat{M}) \wedge x_{ij}=1
\end{cases}
\end{equation}
\begin{equation}
\forall M_i, \nexists M_k, M_j (i \neq k \neq j) \quad\text{satisfying}\quad x_{ik}=1 \wedge x_{ji}=1
\end{equation}
\begin{equation}
\sum\limits_{i=1}^{n}x_{ij}=1
\end{equation}

The above problem is a weighted max-cut problem~\cite{}. If we see each model $M_i$ represents a vertex, and an edge $e_{ij}$ from $M_i$ to $M_j$ specifies to deduplicate $M_j$ using $M_i$ as a base model, while $n_{ij}$ represents the weight of $e_{ij}$. The goal is to find a partition of $\mathcal{M}$ into a set of base models $\mathcal{B}$ and a set of target models $\mathcal{T}$ to maximize the total weights from edges pointing from $\mathcal{B}$ to $\mathcal{T}$. The problem has been proven to be NP-hard~\cite{}.
%If we fix a subset of $m$ models $\mathcal{S}\subset \mathcal{M}$ to be base models, the objective function becomes $\underset{x_{ij}(1 \leq i \leq m,1 \leq j \leq n)}{\max}\sum\limits_{i=1}^{m}\sum\limits_{j=1}^{n}{n_{ij}\times{x_{ij}}}$, where $\mathcal{X}$ becomes a $m\times n$ matrix. Then, the problem is a generalized assignment problem (GAP), where multiple target models (i.e., tasks in the classical GAP problem) are assigned to each base model (i.e., agents in the classical GAP). The GAP problem has been proven to be NP-hard. 
%
In addition, the problem is also a black-box optimization problem~\cite{}, since there is no known ways to estimate $n_{ij}$. Performing actual deduplication to determine $n_{ij}$ requires at least tens of minutes' time for deduplicating a pair of models using a server with 128GB memory and one A10 GPU card, according to our experiences, not to mention the additional privacy costs incurred for accuracy validation. To address the challenges, we developed an effective and dynamic greedy strategy to resolve the problem, described in the next section.
%\noindent
% \textbf{Q3. How will a base model affect the utility?} 
%{\color{blue}A model's performance typically declines as the replacement weights have not been trained in conjunction with other weights. In practice, utility can be managed by establishing a threshold: a deduplication step will be reversed if utility drop exceeds the threshold. Therefore it controls the tradeoff between utility and compression ratio. 

%\noindent
%\textbf{Q4. Can a base model be deduplicated from multiple existing models?} Supposing a base model $\hat{M}$ with privacy budget $\epsilon$, is deduplicated from $\hat{M}_1$ with $\epsilon_1$ and $\hat{M}_2$ with $\epsilon_2$, it must satisfy that $\epsilon = \epsilon_1 + \epsilon_2$ if $\hat{M}_1$ and $\hat{M}_2$ are from the . Typically, $\hat{M}$ has worse utility than source models $\hat{M}_1$ and $\hat{M}_2$ because deduplicating a model usually worsens its utility. It means both $\hat{M}_1$ and $\hat{M}_2$ are a better base model since each of them has a lower privacy budget and a higher utility than $\hat{M}$. Therefore, a base model should not be deduplicated from existing models. 

%Given these trade-offs, we can now analyze the three objectives more closely. Among utility, privacy budget, and compression, we have direct control over the first two during deduplication. The utility objective can be managed by setting a threshold: if deduplicating a block causes a utility drop exceeding this threshold, the step is reversed. Regarding privacy, while it's theoretically possible to involve all models in the deduplication process, this approach is impractical for two reasons. First, the resulting models would all have the same privacy budget and, according to the fairness constraint, should have the same utility. However, the system would not need multiple models with identical privacy budgets and utility on the same dataset, rendering most models redundant. Second, according to Theorem~\ref{privacy-with-deduplication}, the resulting model would have a privacy budget upper bound equal to the sum of all involved models' budgets, potentially many times the original budget. Such a significant increase would severely compromise privacy in practical applications.
%Based on the above analysis, we first introduce a local strategy for base model selection and then generalize it to a global strategy.

%\noindent
%With these questions answered, we are ready to summarize some rules that are useful for the base model selection.
%\begin{align}
%    \epsilon'_j < \epsilon'_k &\iff u'_j < u'_k \label{eq:fairness_dedup} \quad \text{if } M_j \thicksim M_k\\
%    \epsilon_j < \epsilon_k &\iff u_j < u_k \label{eq:fairness_origin} \quad \text{if } M_j \thicksim M_k\\
%    \epsilon_i &\leq \epsilon'_i \label{eq:eps_inc}\\
%    u_i &> u'_i \label{eq:util_drop} \\
%    u_j < u_k &\implies u'_j < u'_k \quad \text{if } M_j \thicksim M_k\label{eq:util_consistency}
%\end{align}
%for any $i,j,k\in\{1,...,n\}$. Eq.~\ref{eq:fairness_origin} and Eq.~\ref{eq:fairness_dedup} are the fairness rule, which applies to both deduplicated models and original models. Eq.~\ref{eq:eps_inc} states that the utility is not less than the original privacy cost (Q1) and the unequality is strict when $R(M_t)=R(\hat{M})$. Eq.~\ref{eq:util_drop} states that the utility drops after deduplication (Q3). A high utility is usually achieved by allocating high privacy budget for training and their utility advantage should be kept after deduplication, which leads to Eq.~\ref{eq:util_consistency}.

%With these rules, we can derive 
% \vspace{-4pt}
%\begin{equation}
%\label{eq:eps_consistency}
%    \epsilon_j<\epsilon_k \implies \epsilon'_j<\epsilon'_k
%\end{equation}
%for any $j,k\in\{1,...,n\}$ because $\epsilon_j<\epsilon_k \overset{Eq.~\ref{eq:fairness_origin}}{\implies} u_j<u_k \overset{Eq.~\ref{eq:util_consistency}}{\implies} u'_j<u'_k \overset{Eq.~\ref{eq:fairness_dedup}}{\implies}  \epsilon'_j<\epsilon'_k$. 
%It says that the ordering of privacy cost is the same before and after dedulication. This is generally true so the privacy constraint should reflect this by ensuring $\epsilon_j < \epsilon_k \implies \epsilon_j+\epsilon^*_j < \epsilon_k+\epsilon^*_k$. 
%}

\begin{comment}
\subsubsection{Local Strategy for Base Model Selection.}
\label{sec:local}
We first focus on deduplicating one model $M_t$. The local strategy aims to iteratively select base models for $M_t$. Each time, it will select one base model $\hat{M}$ for deduplicating $M_t$ with privacy budget $\epsilon_t$ and privacy budget increase constraint $\epsilon^*$. 
We first identify the models that satisfy two criteria: (1) The base model should be the most similar to the target model according to the model's public information (Q2); (2) Its privacy budget $\hat{\epsilon}$ satisfies the following constraints based on Q1:
 




%Easily derived from the above analysis, we will select the most similar model that satisfies the privacy constraint. \review{The following sentences can be more precisely stated.} We first identify base model candidates as $\mathcal{C}=\{\hat{M}_t\}$. Each $\hat{M}_t \in \mathcal{C}$ must have the model architecture, training task, and training dataset as $M_t$ (i.e., according to Q3) and a privacy budget $\hat{\epsilon}_{t}$ satisfying $\hat{\epsilon}_{t} < \min{(\epsilon_{t}, \epsilon^*)}$ (i.e., according to Q2 and Q4's absorbing part). 
 Then, we query top-$k$ candidates that minimize the $\text{distance}(M_t, \hat{M})$ (according to Q2) and select the candidate with the highest utility (according to Q3). The  $\text{distance}$ function uses Euclidean distance of the embedding vectors of models' public attributes, such as model architecture, training data, task, and privacy budget, without introducing aggregated privacy costs. Assuming that the currently selected base model $\hat{M}_{c}$ has a privacy budget of $\hat{\epsilon}_{c}$, the local strategy will update $\epsilon^*$ using Eq.~\ref{eq:eq2} after deduplicating $\hat{M}_c$ and $M_t$. Then it will repeat the process until no qualified base model can be found. %\hong{Check the first equation}
 \vspace{-6pt}
\begin{equation}
\begin{cases}
\label{eq:eq2}
\epsilon^* \leftarrow \epsilon^* - \hat{\epsilon}_{c}  &\text{if}\quad R(\hat{M}_{c}) = R(M_t) \\
\epsilon^* \leftarrow \epsilon^*-(\hat{\epsilon}_{c}- \epsilon_t) &\text{if} \quad R(\hat{M}_{c})  \neq R(M_t) \And \hat{\epsilon}_{c} > \epsilon_t\\
\epsilon^* \leftarrow \epsilon^* &\text{if otherwise}
\end{cases}
\end{equation}
%\hong{Why not just $\hat{\epsilon} < \epsilon_t+\epsilon^*$ but $\max\{\hat{\epsilon}, \epsilon_t \}< \epsilon_t+\epsilon^*$?} 
%Q4 indicates that a base model cannot be derived from a deduplicated model. In addition, the blocks from a base model, once used by a target model $M_t$, if get replaced (i.e., deduplicated) by blocks from another base model, the utility of the $M_t$ will be affected. %Therefore, from a global perspective (i.e., the perspective of the model infrastructure), having many base models will reduce the number of target models that can be deduplicated. 
%Therefore, naively applying the local strategy to each target model may lead to many base models that cannot be deduplicated further and thus hurt the overall compression ratio. In our global strategy, we propose to cluster similar models into a group and make the group share one base model, as detailed in Sec.~\ref{sec:global}.
%\vspace{-25pt}
\end{comment}

\subsubsection{A Greedy Strategy.}
\label{sec:greedy}
Empirically, we have the following intuitions: (\underline{I1}) A base model containing more similar weights to the target model yields a better compression ratio. (\underline{I2}) The quality of the base models is more important than the quantity.  The quality of a base model $M_i$ is defined as the total number of blocks it can deduplicate from other models as base models, subtracting the total number of blocks that can be deduplicated from $M_i$ as a target model, denoted as $\sum\limits_{j=1}^n{n_{ij}\times e_{ij}}-\sum\limits_{j=1}^n{n_{ji}\times e_{ji}}$, where $e_{kl}=1$, if the base model $M_k$ meets $M_l$'s privacy budget increase constraint as defined in Eq.~\ref{eq:problem_constraint}, otherwise, $e_{kl}=0$. (\underline{I3}) Although it is difficult to derive the exact value of $n_{ij}$, one effective heuristic is that using similar base models to deduplicate the same target model (with the same utility drop threshold) leads to similar compression ratios. In addition, among multiple similar candidate base models, the base model with the highest utility usually results in the best compression ratio. %If we set $n_{ij}$ to be a constant $l$ for all $i$ and $j$, which means every pair of base model and target model leads to the same compression ratio of the target model, the optimal solution to the problem would be having only one base model while assigning the rest $n-1$ models to be its target models (i.e., in the matrix $\mathcal{X}$, one row has all ones while other rows have all zeros), resulting in $l\times (n-1)$ blocks to be deduplicated in total.%However, for I1, no known function can directly estimate the compression ratio of deduplicating two models. Although we may use model similarity as an indicator of the compression ratio, checking the similarity between two models based on their weights will aggregate their DP privacy costs, leading to a higher privacy budget for the resulting deduplicated models.
Based on these intuitions, our key ideas include:

\noindent
(1) \textbf{Clustering Models Based on Similarity.} Based on I1, we cluster the models from $\mathcal{M}$ into several groups based on the public information of each model such as model architecture, task, public training dataset, the identifier of the private fine-tuning dataset, and the $\epsilon$. We leveraged a simple hierarchical clustering strategy and ensured that all models in the same group have the same model architecture and are trained for the same task on the same dataset with different $\epsilon$.

\noindent
(2) \textbf{Prioritizing Dangling Models as Base Models.} In each cluster group, we first identify dangling models that do not have any qualified base models (i.e. base models satisfying Eq.~\ref{eq:problem_constraint}). There must be at least one dangling model in each group--the model with the smallest $\epsilon$ in the group, denoted as $M_{min}$. Our key idea is to only allow these dangling models including $M_{min}$ to serve as the base models. Given a target model $M_i$, if $M_{min}$ from the same group does not qualify as $M_i$'s base model, no other models could qualify. Supposing $M_{min}$ qualifies, there may exist one or more non-dangling models from the same group also qualify. However, based on I3, these non-dangling models lead to similar deduplication ratios with $M_{min}$, because they are all from the same similarity group. According to I2, we prioritize the dangling models to be base models, as shown in Alg.~\ref{alg:dangling-models}.

\noindent
(3) \textbf{Intra-Group and Inter-Group Base Model Selection.} Given $M_i$, we will first select the most similar and qualified dangling model from $M_i$'s group as its base model (See line 8 in Alg.~\ref{alg:base-model-main}). If no such model exists, it will search in other cluster groups (See line 9-11 in Alg.~\ref{alg:base-model-main}). 

\begin{algorithm}[t]
\caption{Identify Dangling Models as Candidate Base Models in group $\mathcal{G}=\{M_1, ..., M_k\}$}
\label{alg:dangling-models}
\small
\begin{algorithmic}[1]
\Procedure{CandidateBaseModelGen}{$\mathcal{G}$}
\State  $\mathcal{B}\leftarrow \{\}$; $\mathcal{T}\leftarrow \mathcal{G}$
\For{$M_i$ in $\mathcal{T}$} \Comment{Identify dangling models and add them to $\mathcal{B}$}
    \If{$\epsilon_j \geq \epsilon^{adjusted}_i$ for all $j\in\{1,...,k\}$ and $j\neq i$}
        \State $\mathcal{B} = \mathcal{B} \cup \{M_i\}$;
        \State $\mathcal{T} = \mathcal{T} - \{M_i\}$;
    \EndIf
\EndFor
\State \Return
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{Select a Base Model $M_t$ in a Group $\mathcal{G}$}
\label{alg:base-model-intra}
\small
\begin{algorithmic}[1]
\Procedure{BaseModelSelectStep}{$M_t$, $\mathcal{G}$}
\State $\mathcal{B} \leftarrow $ The set of candidate base models in $\mathcal{G}$; 
\State $\epsilon_{min}$ $\leftarrow$ the epsilon of $M_{min}$
\If{$M_t$ and models from $\mathcal{G}$ are trained on the same dataset}
\If{$\epsilon_{min} \geq \epsilon^{adjusted}_{t}$}
\State \Return NULL;\Comment{No qualified base models found}
\EndIf
\State Find base model $\hat{M} \in \mathcal{B}$ with the largest $\hat{\epsilon}$ to satisfy $\hat{\epsilon} < \epsilon^{adjusted}_t$ to serve as the base model for $M_t$.
\Else
\If{$\epsilon_{min} \geq \epsilon_t+\epsilon^{adjusted}_{t}$} 
\State \Return NULL;\Comment{No qualified base models found}
\EndIf
\State Find base model $\hat{M} \in \mathcal{B}$ with the largest $\hat{\epsilon}$ to satisfy $\hat{\epsilon} < \epsilon_t + \epsilon^{adjusted}_t$ to serve as the base model for $M_t$.
\EndIf
\State \Return $\hat{M}$
%\For{$i$ in $\{|\mathcal{T}|-1,..,1\}$} 
%    \State Find a base model in $\mathcal{B}$ with the largest $\hat{\epsilon}_i$ to satisfies $\hat{\epsilon}_i \leq \epsilon^*_i$ and $\epsilon_i+\hat{\epsilon_i} < \epsilon_{i+1}+\hat{\epsilon}_{i+1}$ to serve as the base model for $M_i$.
%\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
\caption{Base Model Selection for All Models $\mathcal{M}$}
\label{alg:base-model-main}
\small
\begin{algorithmic}[1]
\Procedure{BaseModelSelectMain}{$\mathcal{M}$}
\State $\mathcal{C}=\{\mathcal{G}_1, ..., \mathcal{G}_l\} \leftarrow $ $Cluster(\mathcal{M})$
\For{$\mathcal{G}_i \in  \mathcal{C}$}
\State $CandidateBaseModelGen(\mathcal{G}_i)$
\EndFor
\For{$\mathcal{G}_i \in  \mathcal{C}$}
\State sort ($\mathcal{C}' = \mathcal{C}-\mathcal{G}_i$) based on similarity to $\mathcal{G}_i$
\For{$M_j \in \mathcal{G}_i$}
\State $ret \leftarrow BaseModelSelectStep(M_j, \mathcal{G}_i)$
\While{$ret = NULL$}
\State $\mathcal{G}_k \leftarrow$ next model in $\mathcal{C}'$
\State $ret \leftarrow BaseModelSelectStep(M_j, \mathcal{G}_k)$
\EndWhile
\State record that $M_j$'s base model is $ret$
\EndFor
\EndFor
\Return
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{comment}
\begin{algorithm}[t]
\caption{Intra-Group Base Model Selection}
\label{alg:base-model-intra}
\small
\begin{algorithmic}[1]
\State Sort models in $\mathcal{T}$ in descending order of the privacy budget. 
\State Find base model in $\mathcal{B}$ with the largest $\hat{\epsilon}_{|\mathcal{T}|}$ to satisfy $\hat{\epsilon}_{|\mathcal{T}|} \leq \epsilon^*_{|\mathcal{T}|}$ to serve as the base model for $M_{|\mathcal{T}|}$.
\For{$i$ in $\{|\mathcal{T}|-1,..,1\}$} 
    \State Find a base model in $\mathcal{B}$ with the largest $\hat{\epsilon}_i$ to satisfies $\hat{\epsilon}_i \leq \epsilon^*_i$ and $\epsilon_i+\hat{\epsilon_i} < \epsilon_{i+1}+\hat{\epsilon}_{i+1}$ to serve as the base model for $M_i$.
\EndFor
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
\caption{Inter-data Base Model Selection}
\label{alg:base-model-inter}
\small
\begin{algorithmic}[1]
\State Initialize target models $\mathcal{T}_{d1}$ as all models trained on dataset $d1$ and base models $\mathcal{B}_{d2}$ as all models trained on dataset $d2$.
\State Sort models in $\mathcal{T}_{d1}$ in descending order of the privacy budget.
\State Find a base model in $\mathcal{B}_{d2}$ with the largest $\hat{\epsilon}^{d2}_{|\mathcal{T}|}$ to satisfies $\hat{\epsilon}^{d2}_{|\mathcal{T}|} \leq \epsilon_{|\mathcal{T}|}+\epsilon^*_{|\mathcal{T}|}$ to serve as the base model for $M_{|\mathcal{T}|}$.
\For{$i$ in $\{|\mathcal{T}_{d1}|-1,..,1\}$} 
    \State Find a base model in $\mathcal{B}_{d2}$ with the largest $\hat{\epsilon}^{d2}_i$ to satisfies $\hat{\epsilon}^{d2}_i \leq \epsilon_i+\epsilon^*_i$ and $\max(\hat{\epsilon}^{d2}_i, \epsilon_i+\hat{\epsilon}_i) < \max(\hat{\epsilon}^{d2}_{i+1}, \epsilon_{i+1}+\hat{\epsilon}_{i+1})$ to serve as the base model for $M_i$.
\EndFor
\end{algorithmic}
\end{algorithm}
\end{comment}

\begin{comment}
{\color{blue}
%For simplicity of notation, we first assume each dataset has the same model architecture and extend to multiple model architectures later. 
We denote $\mathcal{G}_d=\{M^d_1,M^d_2,...,M^d_{k}\}$ as a group of $nd$ models trained on dataset $r_d$, $d\in\{1,...,D\}$. To select base models for a target model, every group will run the \textit{base model selection} separately because the privacy cost accounting on disjoint datasets are independent from each other. The union of all the selected models from every group can serve as the base models for this target model. Specifically, Alg.~\ref{alg:base-model-intra} identifies base models within the same group and Alg.~\ref{alg:base-model-inter} identifies base models in inter-data groups.

Line 2-5 of Alg.~\ref{alg:base-model-intra} find the models that no base models can be found to meet the privacy constraint. These base models' privacy costs are unchanged, and according to Eq.~\ref{eq:eps_consistency}, they set a new privacy constraint to other model, making some of them undeduplicatable. Line 6-15 iteratively find such affected models. Lastly, for the remaining models, Line 16-19 find a base model that satisfies $\hat{\epsilon}_i \leq \epsilon^*_i$ (privacy constraint) and $\epsilon_i+\hat{\epsilon_i} < \epsilon_{i+1}+\hat{\epsilon}_{i+1}$ (Eq.~\ref{eq:eps_consistency}). If we allow for multiple base models to deduplicate a single model, we can apply the local strategy to identify multiple models from $\mathcal{B}$ that satisfy the two constraints.
Next, we find base models in other groups. Specifically, for each group, run Alg.~\ref{alg:base-model-inter} over all other groups to identify base models for each pair of groups. Lastly, combine all the models found in Alg.~\ref{alg:base-model-intra} and Alg.~\ref{alg:base-model-inter} as the base models.
If there are multiple model architectures for one dataset, we will prioritize the models with the same architecture within each group because they tends to have more similar weights.

Here, we discuss an alternative algorithm shown in Alg.~\ref{alg:base-model-intra-cascade}. This algorithm allows cascaded deduplication, where a model serve as the target model for one model and the base model for another model. 
% Essentially, it is the local strategy with the fairness rule under consideration.
This cascaded deduplication algorithm has two ways to actually run the deduplication process after base model selection. The first allows keeping a copy of the model even after it is deduplicated and discard the blocks not in any deduplicated model at the very end of the deduplication process. The other does not allow such a model copy and carefully keep track of the blocks that are already deduplicated.
Unfortunetely, both ways have their drawbacks. The first way keeps a copy of all blocks during deduplication and discard the deduplicated blocks at the very end of the deduplication process. This allows any model to be the base model. It can be achieved by skipping two steps of collecting base model in Alg.~\ref{alg:base-model-intra}. This approach can easily result in high compression ratio because some weights in a model are insensitive to changes, so many block used for deduplication when it serves a base model can also be deduplicated when it serves as a target model. Eventually, these blocks are still kept in some models.
The second way does not keep a copy of deduplicated models in the process. There are two cases. If a model first serves as a base model, the blocks used to deduplicate another model can't be deduplicated when it serves as the target model. If it first serves as a target model, the deduplicated model's privacy cost increases (Eq.~\ref{eq:eps_inc}) and may have worse utility than other choice of base models (Eq.~\ref{eq:util_drop}). 
% Therefore, cascaded deduplication is not a good option. 



\begin{algorithm}[t]
\caption{Intra-data Base Model Selection (Cascaded)}
\label{alg:base-model-intra-cascade}
\small
\begin{algorithmic}[1]
\State Sort models in all intra-data models $\mathcal{M}$ in descending order of the privacy budget. 
\State Find base model in $\mathcal{M}$ with the largest $\hat{\epsilon}_{|\mathcal{T}|}$ to satisfy $\hat{\epsilon}_{|\mathcal{T}|} \leq \epsilon^*_{|\mathcal{M}|}$ to serve as the base model for $M_{|\mathcal{M}|}$.
\For{$i$ in $\{|\mathcal{M}|-1,..,1\}$} 
\State Initialize remaining privacy budget for $M_i$ as $\epsilon_{remaining}=\epsilon^*_i$.
\State Initialize base models for $M_i$ as $B_i=\{\}$.
\While{ $\hat{\epsilon}_i \leq \epsilon_{remaining}$}
    \State Find a base model $M_j$ in $\mathcal{M}$ with the largest $\hat{\epsilon}_j$ to satisfies $\hat{\epsilon}_j \leq \epsilon_{remaining}$ and $\epsilon_i+\hat{\epsilon_j} < \epsilon'_{i+1}$ to serve as the base model for $M_i$.
    \State $B_i = B_i \cup \{M_j\}$
    \State $\epsilon_{remaining} = \epsilon_{remaining}-\epsilon_j$
\EndWhile
\State Compute the final privacy budget of the deduplicated model $\epsilon'_i=\epsilon_i+\epsilon^*_i-\epsilon_{remaining}$

\EndFor
\end{algorithmic}
\end{algorithm}

}


%\begin{comment}
{\color{black}
\subsubsection{Deduplication Problem Reduction}
\label{sec:two-model-deduplication}
 The two-model deduplication involves a target model $M_i \in \mathcal{G}$ and a base model $\hat{M}$ selected for $\mathcal{G}$ (i.e., the privacy constraint is guaranteed by base model selection). The optimization objective is to minimize the number of unique blocks in $M'_i$ that are not in $\hat{M}$ (i.e., minimize the compression ratio) while meeting the utility drop constraint formalized below.
%With model groups and base models, the problem is redefined as follows: without loss of generality, assume that the models \(M_1, \dotsc, M_N\) are pre-sorted by their privacy budgets in ascending order. The model \(M_1\) with the smallest privacy budget is set as the base model, and the objective is to find
\begin{gather*}
    \minimize {|\text{UniqueBlocks}(M'_i-\hat{M})|} \text{ with } \\
    M'_i = \text{Deduplicate}(M_i; \hat{M} \text{ as base model}) \;s.t. \\
    u_i-u'_i < T_i 
\end{gather*}
$|\text{UniqueBlocks}(M'_i-\hat{M})|$ represents the set difference of two sets of blocks in $M'_i$ and $\hat{M}$. $T_i$ is derived from the user-specified constraint of utility drop $t^*_i$ (see Sec.~\ref{sec:formulation}) to enforce $u_i - u'_i < t^*_i$ and the fairness constraint. 
%First, the fairness requirement will be violated if two target models using the same dataset and model architecture overlap in their allowed accuracy ranges. %For example, if $M_i$'s utility is smaller than $M_j$'s, denoted as $u_i<u_j$, and $u_i-t^*_i<u_j-t^*_j < u_i$, then there is an overlap in their ranges, which is $[u_i-t^*_i, u_j]$. It is possible that the deduplicated models' utilities $u'_j,u'_k$ fall in this overlapping range and $u'_j>u'_k$, which violates the fairness rule.  
We sort these models governed by the same fairness constraint (i.e., models trained on the same dataset with the same model architecture for the same task) according to the beginning of their utility ranges $[u_i-t^*_i, u_i]$ in ascending order. Then, we deduplicate the models sequentially, setting the threshold $T_i$ based on the previous deduplicated model's utility ($u'_{i-1}$), following Eq.~\ref{eq1}.
%to the maximum of the previous deduplicated model's utility $u'_{i-1}$ and $t_i$, as defined in Eq.~\ref{eq1}.
\vspace{-5pt}
\begin{equation}
\label{eq1}
    T_i = \min(u_i-u'_{i-1}, t^*_i) \text{ for } M_i 
\end{equation}
}
 To meet the ordering constraint, we schedule these tasks following a total ordering identified by applying the topology sort algorithm~\cite{knuth1997art} on the nodes of a directed acyclic graph, of which nodes represent models and directed edges represent base-model and target-model relationships assigned by the global strategy. 
\end{comment}
